Enhancing and Assessing Instruction-Following with Fine-Grained Instruction Variants

The effective alignment of Large Language Models (LLMs) with precise instructions is essential for their application in diverse real-world scenarios. Current methods focus on enhancing the diversity and complexity of training and evaluation samples, yet they fall short in accurately assessing LLMs' ability to follow similar instruction variants. We introduce an effective data augmentation technique DeMoRecon that decomposes complex instructions into simpler sub-components, modifies these, and reconstructs them into new variants, thereby preserves the original instruction's context and complexity while introducing variability, which is critical for training and evaluating LLMs' instruction-following precision. Based on DeMoRecon, we developed the FGIV dataset which contains fine-grained instruction variants of 1,773 seed instructions to both fine-tune and evaluate LLMs. Our findings show that LLMs fine-tuned with FGIV will gain significant performance boost on both ours and commonly used instructions-following benchmarks.

==> section/1-intro_backup.tex <==
\section{Introduction}
\label{sec:intro}
The ascent of Large Language Models (LLMs) has transformed many Natural Language Processing (NLP) tasks into challenges centered around natural language generation, exploiting the advanced understanding capabilities of these models. While the initial strategies in prompt engineering have shown promise, deploying LLMs broadly in real-world applications has revealed critical issues, especially in their adherence to intricate instructions.

To tackle these issues, novel approaches such as instruction tuning and alignment tuning have been developed. Instruction tuning \citep{instruction-tuning}, for instance, trains LLMs using high-quality instruction-response pairs. The study by \citet{LIMA} demonstrates this by fine-tuning models with only 1,000 such pairs, highlighting the importance of the quality and diversity of instructions. Moreover, the Evol-Instruct technique by \citet{wizardLM} advances this by evolving simple instructions into more complex variants through iterative interactions with ChatGPT, leading to notable performance gains across various benchmarks.

On the other hand, alignment tuning \citep{RLHF} methods like DPO \cite{DPO} and KTO \cite{KTO} aim to refine models' ability to discern between effective and ineffective responses, aligning more closely with human preferences. A notable implementation of this method is seen in the work of \citet{conifer}, who employed GPT-4 for generating intricate instructions and used DPO for fine-tuning, setting new standards in instruction-following tasks.

Despite these advancements, most efforts have concentrated on enhancing the complexity and diversity of instructions, overlooking the ability of LLMs to discern subtle differences in instructions at a finer granularity. This gap is also evident in current benchmarks that assess the instruction-following capabilities of LLMs. Existing benchmarks typically focus on rule-based formats \citep{IFEval}, test LLMs with progressively challenging instructions \citep{FollowBench}, or assess instruction-following at a granular level for reliability and interpretability \citep{InFoBench}. However, these benchmarks often fail to capture the nuances within instructions of similar difficulty and context, where only minor variations in sub-instructions occur. This oversight underscores a critical gap in our assessment methods, highlighting the need for developing evaluation metrics that can detect these finer nuances in instruction understanding. Such metrics would enable a more detailed analysis of LLMs' comprehension and execution capabilities for subtly varied instructions, offering deeper insights into model performance and facilitating more targeted refinements in instruction-based training.


To address these shortcomings, we propose a effective method that augments instructions into similar variants by decomposing each instruction into sub-instructions, modifying them, and then reconstructing these into new variants that maintain the same difficulty level and context. Leveraging this approach, we developed the \dataname datasets to both enhance and evaluate instruction-following capabilities. Specifically, \dataname-Aug utilizes direct responses from GPT-4 based on the augmented instructions for training purposes. In contrast, \dataname-Ref employs responses revised from the original dataset to ensure maximum similarity with the original instructions. Meanwhile, \dataname-Eval, comprising 170 instructions and their augmentations, uses GPT-4 to assess the accuracy of instruction following.

Our evaluation of the \dataname dataset's efficacy in enhancing the instruction-following capabilities of LLMs involves using both instruction tuning and alignment tuning on pre-tuned LLMs, assessing their performance across \dataname-Eval and established benchmarks like IFEval \citep{IFEval}, InfoBench \citep{InFoBench}, and FollowBench \citep{FollowBench}. The results indicate significant improvements in LLMs' ability to follow instructions accurately. The key contributions of our work are as follows:
\begin{itemize}
    \item {We introduce a data augmentation method that breaks down complex instructions into simpler sub-components, modifies them, and reassembles them into new variants. This preserves the original instruction's difficulty and context while increasing variability, thereby improving LLMs’ ability to detect nuanced differences in commands. }

    \item{We develop the \dataname dataset, which includes three components (\dataname-Aug, \dataname-Ref, and \dataname-Eval), targeting both enhanced training and rigorous evaluation of LLMs' instruction-following abilities. This dataset is specifically designed to test LLMs on subtle variations within instructions, providing a refined tool for assessing nuanced comprehension and execution.}
    
    \item{Through comprehensive testing, we show that LLMs trained with \dataname outperform those trained with traditional benchmarks in nuanced instruction-following tasks. Our findings, validated using several leading LLMs including GPT-4, establish \dataname as a critical benchmark for future assessments in this field. We have made the training data and source code fully open-source to support ongoing research.}
\end{itemize}




==> table/all_bu.tex <==
\begin{table*}[]
\small
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{cclcccccc|ccc}\toprule
\multicolumn{3}{c}{\multirow{2}{*}{Model}}                                                                                                    & \multicolumn{6}{c|}{FollowBench (HSR)}                                                              & \multicolumn{3}{c}{InfoBench}  \\ \cmidrule{4-12} 
\multicolumn{3}{c}{}                                                                                                                          & Level 1        & Level 2        & Level 3        & Level 4        & Level 5        & Avg.           & Easy  & Hard  & Average        \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{LLaMA-2-7B-Chat}}     & \multicolumn{2}{c|}{Original}                                                     & 57.68          & 51.96          & 38.16          & 36.02          & 31.67          & 43.10           & 79.57 & 76.60  & 77.51          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{3}{*}{SFT}}     & \multicolumn{1}{l|}{Plain}        & 61.55          & 51.51          & 41.85          & \textbf{38.67} & 28.86          & 44.49          & \textbf{84.20}  & 76.28 & 78.71          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Augmentation} & 57.31          & 50.91          & 44.07          & 36.02          & 31.78          & 44.02          & 81.88 & 77.31 & 78.71          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 59.74          & 51.68          & 42.54          & 36.58          & 25.89          & 43.28          & 81.88 & 73.59 & 76.13          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{2}{*}{SFT+DPO}} & \multicolumn{1}{l|}{Augmentation} & 61.23          & 55.18          & 43.31          & 36.93          & 31.17          & 45.56          & 82.61 & 78.91 & 80.04          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & \textbf{63.29} & \textbf{56.38} & \textbf{44.41} & 34.95          & \textbf{33.00}    & \textbf{46.41} & 82.17 & \textbf{80.58} & \textbf{81.07} \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{Qwen1.5-7B-Chat}}     & \multicolumn{2}{c|}{Original}                                                     & 74.35          & 58.80           & 52.85          & 44.66          & 34.33          & 53.00             & 84.49 & 78.85 & 80.58          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{3}{*}{SFT}}     & \multicolumn{1}{l|}{Plain}        & 70.42          & \textbf{61.57} & 51.77          & 42.66          & \textbf{40.37} & 53.36          & 83.62 & 77.37 & 79.29          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Augmentation} & 69.17          & 58.55          & 48.37          & 43.33          & 36.03          & 51.09          & 84.93 & 77.47 & 79.73          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & \textbf{73.75} & 57.34          & 55.23          & 42.58          & 34.96          & 52.77          & 85.07 & 75.90  & 78.71          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{2}{*}{SFT+DPO}} & \multicolumn{1}{l|}{Augmentation} & 70.22          & 59.69          & 50.72          & 37.89          & 38.29          & 51.36          & 84.93 & \textbf{79.42} & \textbf{81.11} \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 69.64          & \textbf{61.57} & \textbf{57.36} & \textbf{47.98} & 37.75          & \textbf{54.86} & \textbf{86.09} & 78.78 & 81.02          \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{Mistral-7B-Instruct}} & \multicolumn{2}{c|}{Original}                                                     & 61.70           & 52.29          & 40.92          & 34.18          & 23.67          & 42.55          & 85.22 & 76.47 & 79.16          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{3}{*}{SFT}}     & \multicolumn{1}{l|}{Plain}        & \textbf{61.52} & 50.44          & 47.09          & 39.82          & 33.93          & 46.56          & 84.64 & 75.26 & 78.13          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Augmentation} & 59.63          & 55.77          & 47.18          & 40.40           & 32.94          & 47.18          & 84.35 & 75.71 & 78.36          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 61.06          & 53.95          & 48.14          & 37.93          & 30.77          & 46.37          & 83.77 & 76.35 & 78.62          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{2}{*}{SFT+DPO}} & \multicolumn{1}{l|}{Augmentation} & 60.46          & 56.50           & \textbf{49.38} & \textbf{45.76} & \textbf{36.02} & \textbf{49.63} & \textbf{85.65} & 76.92 & 79.60           \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 59.27          & \textbf{56.93} & 48.45          & 41.93          & 31.80           & 47.68          & 84.64 & \textbf{78.78} & \textbf{80.58} \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{LLaMA-2-13B-Chat}}    & \multicolumn{2}{c|}{Original}                                                     & 56.36          & 54.74          & 45.31          & 37.80           & 30.49          & 44.94          & 83.91 & 79.81 & 81.07          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{3}{*}{SFT}}     & \multicolumn{1}{l|}{Plain}        & 60.28          & 53.03          & 42.59          & \textbf{41.94} & 34.96          & 46.56          & 83.91 & 79.68 & 80.98          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Augmentation} & 59.95          & 51.67          & 43.28          & 39.11          & 35.26          & 45.85          & 84.49 & 79.04 & 80.71          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 59.72          & 54.08          & 45.35          & 39.30           & \textbf{35.52} & 46.79          & 84.93 & 79.49 & 81.16          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{2}{*}{SFT+DPO}} & \multicolumn{1}{l|}{Augmentation} & \textbf{64.79} & 53.91          & 46.35          & 41.39          & 29.73          & 47.23          & \textbf{86.38} & \textbf{81.28} & \textbf{82.84} \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 61.22          & \textbf{55.40}  & \textbf{47.88} & 40.51          & 35.33          & \textbf{48.07} & 86.09 & 80.17 & 82.36          \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{Qwen1.5-14B-Chat}}    & \multicolumn{2}{c|}{Original}                                                     & 76.99          & 60.19          & 57.81          & 45.31          & 36.32          & 55.32          & 84.49 & 81.54 & 82.44          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{3}{*}{SFT}}     & \multicolumn{1}{l|}{Plain}        & 67.87          & 55.85          & 49.77          & 43.01          & 33.95          & 50.09          & 83.48 & 79.55 & 80.76          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Augmentation} & 67.17          & 58.04          & 52.33          & 47.05          & 35.69          & 52.05          & 82.75 & 79.55 & 80.53          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 71.99          & 55.98          & 54.59          & 43.17          & 33.92          & 51.93          & 84.20  & 77.05 & 79.24          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{2}{*}{SFT+DPO}} & \multicolumn{1}{l|}{Augmentation} & \textbf{79.81} & \textbf{65.28} & \textbf{59.00}    & 48.94          & 37.06          & \textbf{58.02} & \textbf{86.09} & 82.12 & \textbf{83.33} \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 77.42          & 60.37          & 51.99          & \textbf{49.45} & \textbf{42.00}    & 56.25          & 85.36 & \textbf{82.31} & 83.24          \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{Orion-14B-Chat}}      & \multicolumn{2}{c|}{Original}                                                     & 69.42          & 57.81          & 41.97          & 27.65          & 23.73          & 44.12          & 83.33 & 73.33 & 76.40           \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{3}{*}{SFT}}     & \multicolumn{1}{l|}{Plain}        & 66.54          & 55.87          & 45.43          & 45.13          & 31.09          & 48.81          & 82.03 & 73.46 & 76.09          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Augmentation} & 69.08          & 55.59          & 48.51          & 42.53          & 30.13          & 49.17          & 83.19 & 74.36 & 77.07          \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 67.32          & 56.72          & 45.75          & 40.93          & 32.83          & 48.71          & 82.32 & 71.22 & 74.62          \\ \cmidrule{2-3}
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{\multirow{2}{*}{SFT+DPO}} & \multicolumn{1}{l|}{Augmentation} & \textbf{73.78} & 60.85          & 52.99          & \textbf{45.18} & 35.29          & 53.62          & 84.35 & \textbf{76.28} & \textbf{78.76} \\
\multicolumn{1}{c|}{}                                     & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Reference}    & 73.44          & \textbf{61.25} & \textbf{53.48} & 43.54          & \textbf{38.27} & \textbf{54.00}    & \textbf{85.07} & 75.90  & 78.71         \\\bottomrule  
\end{tabular}
\end{adjustbox}
\caption{Full experimental results on FollowBench (HSR) and InfoBench.}
\label{tab-all}
\end{table*}

==> table/benchmark_bu.tex <==
\begin{table}[t]
\small
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l|cccccc}\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{6}{c}{FGIV-Eval}                                                          \\ \cmidrule{2-7} 
\multicolumn{1}{c|}{}                       & Ori    & Seed & Aug & Ref & FGIV-A   & FGIV-R      \\ \midrule
GPT-4                                       & 95.00                    & -          & -          & - & - & - \\
GPT-4-Ref                                   & 91.03                     & -          & -          & - & - & -  \\ \hline
Llama2-7B-Chat                             & 54.71                     & 56.32          & 59.12          & {59.26} & {60.29} & \textbf{60.44} \\
Qwen1.5-7B-Chat                            & 61.91                     & {71.03} & 70.74          & 69.56          & \textbf{72.06} & 70.59          \\
Mistral-7B-Instruct                        & 64.41                     & 66.32          & 67.79          & {68.24} & 67.79          & \textbf{71.18} \\
Llama2-13B-Chat                            & 58.82                     & 62.56          & 64.12          & {63.38} & 64.41          & \textbf{65.15} \\
Qwen1.5-14B-Chat                           & 73.53                     & 72.06          & {76.32} & 73.97          & 79.26          & \textbf{81.62} \\
Orion-14B-Chat                             & 56.62                     & 62.21          & {67.06} & 66.03          & \textbf{68.82} & 68.38          \\\midrule
                                           & \multicolumn{6}{c}{FollowBench (average HSR)}                                                        \\\midrule
Llama2-7B-Chat                             & 43.10                      & 44.49          & 44.02          & 43.28          & 45.56          & \textbf{46.41} \\
Qwen1.5-7B-Chat                            & 53.00                        & 53.36          & 51.09          & 52.77          & 51.36          & \textbf{54.86} \\
Mistral-7B-Instruct                        & 42.55                     & 46.56          & 47.18          & 46.37          & \textbf{49.63} & 47.68          \\
Llama2-13B-Chat                            & 44.94                     & 46.56          & 45.85          & 46.79          & 47.23          & \textbf{48.07} \\
Qwen1.5-14B-Chat                           & 55.32                     & 50.09          & 52.05          & 51.93          & \textbf{58.02} & 56.25          \\
Orion-14B-Chat                             & 44.12                     & 48.81          & 49.17          & 48.71          & 53.62          & \textbf{54.00}    \\\midrule
                                            & \multicolumn{6}{c}{InfoBench (average)}                                                                  \\ \midrule
Llama2-7B-Chat                              & 77.51                     & 78.71 & 78.71        & 76.13     & 80.04          & \textbf{81.07} \\
Qwen1.5-7B-Chat                             & 80.58                     & 79.29 & 79.73        & 78.71     & \textbf{81.11} & 81.02          \\
Mistral-7B-Instruct                         & 79.16                     & 78.13 & 78.36        & 78.62     & 79.60           & \textbf{80.58} \\
Llama2-13B-Chat                             & 81.07                     & 80.98 & 80.71        & 81.16     & \textbf{82.84} & 82.36          \\
Qwen1.5-14B-Chat                            & 82.44                     & 80.76 & 80.53        & 79.24     & \textbf{83.33} & 83.24          \\
Orion-14B-Chat                              & 76.40                     & 76.09 & 77.07        & 74.62     & \textbf{78.76} & 78.71          \\ \midrule
                                            & \multicolumn{6}{c}{IFEval (loose prompt)}                                                                     \\ \midrule
Llama2-7B-Chat                              & 45.84                     & 44.18 & 43.99        & 46.95     & \textbf{49.17} & \textbf{49.17} \\
Qwen1.5-7B-Chat                             & 43.62                     & 47.50  & 44.92        & 46.95     & 45.47          & \textbf{51.02} \\
Mistral-7B-Instruct                         & 43.25                     & 42.51 & 45.84        & 45.66     & 47.69          & 48.24          \\
Llama2-13B-Chat                             & 48.06                     & 46.77 & 49.17        & 48.24     & 51.39          & \textbf{52.31} \\
Qwen1.5-14B-Chat                            & 47.87                     & 39.93 & 39.74        & 44.36     & 55.45          & \textbf{56.75} \\
Orion-14B-Chat                              & 37.89                     & 36.60  & 40.67        & 38.26     & \textbf{53.05} & 50.09    
\\\bottomrule     
\end{tabular}
\end{adjustbox}
\caption{Experimental results on FGIV-Eval and other instruction-following benchmarks. The performance of the official chat LLMs are recorded under ``Ori''.}
\label{tab_bechmark}
% \vspace{-5mm}
\end{table}


==> table/result.tex <==
\begin{table*}[h]
%The values in bracket indicate the performance improvement achieved by fine-tuning with instructions generated by IF, as compared to the use of \texttt{evol-codealpaca-v1} alone.}
\small
\centering
\begin{tabular}{l|c c c c| c c}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}}&\multicolumn{4}{c|}{SFT}  &\multicolumn{2}{c}{DPO+SFT}  \\
 &Original &Plain &Augmentation &Reference & Augmentation &Reference \\\midrule
    GPT4-Turbo
    &95.00&-&-&-&-&-\\
    GPT4-Turbo-Ref
    &91.03&-&-&-&-&-\\
\midrule
    Llama2-7B-Chat
    &54.71 & 56.32          & 59.12          & \textbf{59.26} & \textbf{60.29} & \textbf{60.44} \\
    Qwen1.5-7B-Chat
    &64.41 & 66.32          & 67.79          & \textbf{68.24} & 67.79          & \textbf{71.18} \\
    Mistral-7B-Instruct
    &61.91 & \textbf{71.03} & 70.74          & 69.56          & \textbf{72.06} & 70.59          \\
\midrule
    Llama2-13B-Chat
    &58.82 & 62.56          & 64.12          & \textbf{63.38} & 64.41          & \textbf{65.15} \\
    Qwen1.5-14B-Chat
    &73.53 & 72.06          & \textbf{76.32} & 73.97          & 79.26          & \textbf{81.62} \\
    Orion-14B-Chat
    &56.62 & 62.21          & \textbf{67.06} & 66.03          & \textbf{68.82} & 68.38  \\
\bottomrule 
\end{tabular}
\caption{Experimental results on FGIV-Eval.}
\label{tab-python}
% \vspace{-5mm}
\end{table*}
